Fredman's Trick Meets Dominance Product: Fine-Grained Complexity of Unweighted APSP, 3SUM Counting, and More

In this paper we carefully combine Fredman's trick [SICOMP'76] and Matou\v{s}ek's approach for dominance product [IPL'91] to obtain powerful results in fine-grained complexity: - Under the hypothesis that APSP for undirected graphs with edge weights in $\{1, 2, \ldots, n\}$ requires $n^{3-o(1)}$ time (when $\omega=2$), we show a variety of conditional lower bounds, including an $n^{7/3-o(1)}$ lower bound for unweighted directed APSP and an $n^{2.2-o(1)}$ lower bound for computing the Minimum Witness Product between two $n \times n$ Boolean matrices, even if $\omega=2$, improving upon their trivial $n^2$ lower bounds. Our techniques can also be used to reduce the unweighted directed APSP problem to other problems. In particular, we show that (when $\omega = 2$), if unweighted directed APSP requires $n^{2.5-o(1)}$ time, then Minimum Witness Product requires $n^{7/3-o(1)}$ time. - We show that, surprisingly, many central problems in fine-grained complexity are equivalent to their natural counting versions. In particular, we show that Min-Plus Product and Exact Triangle are subcubically equivalent to their counting versions, and 3SUM is subquadratically equivalent to its counting version. - We obtain new algorithms using new variants of the Balog-Szemer\'edi-Gowers theorem from additive combinatorics. For example, we get an $O(n^{3.83})$ time deterministic algorithm for exactly counting the number of shortest paths in an arbitrary weighted graph, improving the textbook $\widetilde{O}(n^{4})$ time algorithm. We also get faster algorithms for 3SUM in preprocessed universes, and deterministic algorithms for 3SUM on monotone sets in $\{1, 2, \ldots, n\}^d$.

==> counting_table.tex <==
\begin{table*}[ht]
\centering
\begin{tabular}{|cc|c|c|c|}
\hline
    \multicolumn{2}{|c|}{Problems} & References &  Deterministic & Work for Reals\\
    \hline
    \MinPlus{} & & Thm.~\ref{thm:minplus-count} + Thm.~\ref{?} &  & \checkmark \\
    \hline
    \AEExactTri{} & & Thm.~\ref{thm:exact-tri-count} & \checkmark & \checkmark \\
    \hline
    \ExactKClique{} & & Thm.~\ref{thm:exact-k-clique-counting} & \checkmark & \checkmark \\
    \hline
    \MinKClique{} & & Thm.~\ref{thm:min-k-clique-counting}+Thm.~\ref{?} &  & \checkmark \\
    \hline
    \ThreeSUMConv{} & & Thm.~\ref{thm:all-3sum-conv-count} &  & \checkmark \\
    \hline
    \MinPlusConv{} & & Thm.~\ref{thm:minplus-conv-count} + Thm.~\ref{?} &  & \checkmark \\
    \hline
    \AllThreeSUM{} & & Thm.~\ref{thm:all-3sum-count} & & \\
    \hline
    \MonoConv{} & & Thm.~\ref{thm:mono-conv-count} & & \\
    \hline
    \APSP{} & $\dag$ & Thm.~\ref{thm:apsp-count-mod} & \checkmark & \checkmark\\
    \hline
\end{tabular}
\caption{This table summarizes the list of problems whose counting version is shown to be equivalent to its detection version. For \APSP{}, we only show its equivalence to \APSPCountMod{c} for $O(\log n)$-bit integers $c \ge 2$.}
\end{table*}
